BayBFed: Bayesian Backdoor Defense for Federated Learning

Federated learning (FL) allows participants to jointly train a machine learning model without sharing their private data with others. However, FL is vulnerable to poisoning attacks such as backdoor attacks. Consequently, a variety of defenses have recently been proposed, which have primarily utilized intermediary states of the global model (i.e., logits) or distance of the local models (i.e., L2-norm) from the global model to detect malicious backdoors. However, as these approaches directly operate on client updates, their effectiveness depends on factors such as clients' data distribution or the adversary's attack strategies. In this paper, we introduce a novel and more generic backdoor defense framework, called BayBFed, which proposes to utilize probability distributions over client updates to detect malicious updates in FL: it computes a probabilistic measure over the clients' updates to keep track of any adjustments made in the updates, and uses a novel detection algorithm that can leverage this probabilistic measure to efficiently detect and filter out malicious updates. Thus, it overcomes the shortcomings of previous approaches that arise due to the direct usage of client updates; as our probabilistic measure will include all aspects of the local client training strategies. BayBFed utilizes two Bayesian Non-Parametric extensions: (i) a Hierarchical Beta-Bernoulli process to draw a probabilistic measure given the clients' updates, and (ii) an adaptation of the Chinese Restaurant Process (CRP), referred by us as CRP-Jensen, which leverages this probabilistic measure to detect and filter out malicious updates. We extensively evaluate our defense approach on five benchmark datasets: CIFAR10, Reddit, IoT intrusion detection, MNIST, and FMNIST, and show that it can effectively detect and eliminate malicious updates in FL without deteriorating the benign performance of the global model.

==> 000_MR_Requirement.tex <==

{\centering \section*{SUMMARY OF CHANGES}}
\noindent\answer{We thank the reviewers for their insightful comments and constructive feedback.
%, which has helped us better communicate the core aspects and technical contributions of our proposed \ourname approach and improve the overall quality of the paper. 
We have made significant changes to the paper as follows: 
\begin{itemize}

\item We addressed all requirements for the major revision outlined by the reviewers. 

\item Further, we have also addressed all questions and comments raised by the individual reviewers and have added the corresponding explanations. 

\item In addition, we have conducted several new experiments showing the effectiveness of \ourname on further datasets (MNIST, FMNIST), as well as against another, adaptive attack strategy to provide additional information as requested by the reviewers. 
\item We also improved the quality of our writing. 

\end{itemize}

%Below, we first provide a detailed breakdown of the changes made to the manuscript to address the detailed major revision requirements set forth by the reviewers. 

%After that, we provide detailed responses and outline the changes that were undertaken to address the other questions and comments raised by the individual reviewers in their reviews.\\
%on what changes in the manuscript we have made to satisfy the expected explicit requirements for the major revision. 
%And then, we present our detailed responses to the questions and comments raised by individual reviewers in their reviews. \\

\textbf{Note}: Our answers/explanations are marked in \answer{green} color, whereas changes to the manuscript text are typeset in \changed{blue}.} \\


\section{EXPECTATIONS FOR MAJOR REVIEW}
\noindent\answer{In response to the major revision requirements provided by the reviewers, we have revised our paper to include clarifications and additional experimental results to address all nine explicit major revision requirements R1 to R9.}\\
%\commentAS{There are 9 requirements R1 to R9}\\


\textbf{R1.} Justify or tone down the following claim "This defense is relevant in a general adversarial model setting, i.e., it is not conditionally dependent on the attack strategy of the adversary, the underlying data distributions of benign and adversarial datasets, and the selected clients in each training round." \\
\answer{Based on the reviewer's comments, we decided to omit the word "decoupling" to avoid any misinterpretation with independency, Instead, we reformulate our claim and explain what we meant by decoupling, as follows: the existing defense mechanisms works \emph{directly} on the clients' updates; thus their defense accuracy is dependent on multiple factors, such as the clients' data-distribution, an adversary's attack strategy or the number of client's selected in an FL round. Thus, our motivation in this work is to create an alternate, more generic representation of client updates that can accommodate any changes being made in the client updates due to any local client's training strategy. Hence, \ourname computes a probabilistic measure over the clients' updates to keep track of any adjustments made in the updates, and uses a novel detection algorithm that can leverage this probabilistic measure to efficiently detect and filter out malicious updates. Thus, it overcomes the shortcomings of previous approaches that arise due to the \emph{direct} usage of client updates; nevertheless, our probabilistic measure will include all aspects of the local client training strategies. Thus, as requested by the reviewers, we reformulated our claim in the Abstract, Introduction (\sect\ref{sec:introduction}), and Conclusion (\sect\ref{sec:conclusion}):}\\ 
%have toned down the claim that \ourname is independent of the attack strategy of the adversary, the underlying data distributions of benign and adversarial datasets, and the selected clients in each training round. 
%Our motivation is to leverage the computed probabilistic measure (Beta process posterior) to make %\commentAS{you still did not explain what decouple means}
%the \textbf{detection part} of the defense independent (decoupled) from the clients’ training, data distribution, and the number of clients selected in a training round. Here, by decoupling, we mean that we are disassociating the functioning of the detection or the clustering algorithm from any local client's training strategy as it does not administer the client's weights directly. Hence, \ourname is not completely decoupled from the above factors, just the detection algorithm. Specifically, we have made the following changes in the Abstract (page 14), Introduction (page 15), and Conclusion (page 30) sections:}\\
\answer{Abstract:} \changed{In this paper, we introduce a novel and %completely different approach and present a 
more generic backdoor detection framework, called \ourname, which employs a completely different approach of utilizing probability distributions over client updates to detect malicious updates in FL: 
%against backdoor attacks in FL that utilizes Bayesian non-parametric (BNP) modeling techniques. 
\ourname computes a probabilistic measure over the clients' updates to keep track of any adjustments made in the updates, and uses a novel detection algorithm that can leverage this probabilistic measure to efficiently detect and filter out malicious updates. Thus, it overcomes the shortcomings of previous approaches that arise due to the \emph{direct} usage of client updates; nevertheless, our probabilistic measure will include all aspects of the local client training strategies.} \\% \changed{It functions in two steps. First, it computes an (alternate) probabilistic measure over the clients' weights to keep track of their deviations. Second, a detection algorithm leverages this probabilistic measure to decouple itself %\commentAS{decouple? cannot you find another word?} 
 %(making itself independent) from the aforementioned assumptions, as it does not have to administer the client weights \textit{directly}.}\\
\answer{Introduction:} \changed{Moreover, current state-of-the-art defenses against backdoor attacks make several assumptions about the underlying data and the adversary's adopted strategies, as well as they \emph{directly} employ client weights during detection. In this context, we  encountered two main open challenges: First, how can we
%The first one concerns the question of whether we can 
compute an alternate, more generic, representation of client weights (or updates), such as a probabilistic measure, which will encompass all adjustments made to the client updates due to any local client's training strategy. Second, can we design of an efficient detection/clustering algorithm that can leverage such a probabilistic measure to effectively filter out malicious updates in FL, without deteriorating the benign accuracy of the global model. We intuitively believe, and later empirically show, that designing a detection algorithm with such a generic probabilistic measure as one of its inputs provides several significant advantages over existing defense solutions. First, different local client training strategies will not affect the detection process at the global server. Consequently, the defense mechanism's detection phase will remain agnostic about an adversary's attack strategies. Second, utilizing distributions over client updates in the defense instead of directly employing client weights makes the detection process relatively uninfluenced by the underlying local data distributions used for training. }\\%\changed{The first challenge is, how to compute an alternate representation of the client weights (probabilistic measure) that will represent the deviations made in the client weights. Thus, can be effectively used to decouple the detection/clustering part of the defense, i.e., detection of the malicious updates from any operations transpired on the client, such as adversarial training, different data distributions, or the number of clients selected in a training round? Here, by decoupling, we mean that we are disassociating the functioning of the detection or clustering algorithm from any local client's training strategy as it does not employ the client's weights directly.} \\
%\changed{This defense is relevant in the most adversarial model setting, i.e., as we are trying to decouple the detection/clustering function of the defense from the attack strategies of an adversary, the underlying data distributions of the local clients, and the selected clients in each training round.} \\
\answer{Conclusion:}
\changed{This paper proposes \ourname, a novel and more generic probabilistic approach to defend against backdoor attacks in Federated Learning. 
In contrast to existing defenses that mainly consider models as a set of vectors and matrices~\cite{blanchard17Krum,fung2020FoolsGold,mcmahan2018iclrClipping,munoz19AFA,nguyen22Flame,shen16Auror} and operate \emph{directly} on them, \ourname first computes a probabilistic measure over the clients' updates that encompass all the adjustments made in the updates due to any local client training strategy. Then, \ourname employs a detection algorithm that utilizes this probabilistic measure to detect and filter out malicious updates. Thus, it overcomes several shortcomings of previous backdoor defense approaches. \ourname utilizes two extensions of Bayesian non-parametric modeling techniques: the Hierarchical Beta-Bernoulli Process to draw a probabilistic measure given the clients' model updates (or weights), and a variation of the Chinese Restaurant Process, CRP-Jensen, which is a clustering algorithm that can leverage the probabilistic measure to detect and filter out malicious updates. Our extensive evaluation with benchmark datasets in different domains demonstrates that \ourname effectively can mitigate backdoor attacks in FL while preserving the \mbox{benign performance of the global model.} } \\


\textbf{R2.} Justify or tone down the following claim "To the best of our knowledge, all existing defenses consider the model updates as a set of vectors and matrices and directly administer these weights to filter out the malicious client updates."\\
\answer{Different defenses have been proposed in the literature for Federated Learning (FL). However, all these defense proposals make different assumptions and focus on different scenarios. For example, some defenses assume benign models to be similar and outlier models to be poisoned~\cite{nguyen22Flame,blanchard17Krum,munoz19AFA} while other defenses assume poisoned models to be similar and benign models to differ from each other~\cite{fung2020FoolsGold}. These defenses consider the model updates mainly as vectors, where they apply vector operations, such as computation of cosine angular distance~\cite{munoz19AFA,nguyen22Flame,fung2020FoolsGold}, or euclidean distance~\cite{mcmahan2018iclrClipping,nguyen22Flame,blanchard17Krum}, apply clustering on the numbers of these vectors~\cite{shen16Auror}, evaluate predictions of the models using test data~\cite{rieger2022deepsight,andreina2020baffle}, or determine the median of the parameters~\cite{yin2018byzantine}. In comparison, \ourname is, to the best of our knowledge, the first defense that considers the updates to be drawn from random distributions (depending on their training data) for identifying poisoned model updates. We have clarified this in \sect\ref{sec:introduction} (Introduction), as outlined below:}\\
\changed{To the best of our knowledge, existing defenses mainly consider the model updates as a set of vectors and matrices, and \emph{directly} administer these weights to filter out the malicious client updates~\cite{nguyen22Flame,blanchard17Krum,fung2020FoolsGold,shen16Auror,munoz19AFA,mcmahan2018iclrClipping}. Given the client weights, \ourname first estimates a probabilistic measure (such as the Beta posterior) that accurately captures the variations in the clients' weights and then uses a novel clustering technique based on the Chinese Restaurant Process and Jensen-Divergence for identifying the poisoned models.} \\

\textbf{R3.} Include details requested by reviewer D during the discussion (including the 2nd algorithm) and its justification in the paper (under Section 5.3). \\
\answer{We have extended the \ourname workflow by adding the $DetectFilter$ algorithm in \sect\ref{sec:rationale}. $DetectFilter$ is the same approach that we have used throughout the paper for detecting malicious updates, but we have now presented it more formally in the paper. Each round of this algorithm takes the maximum \jensenDivergence of each client stored in an array $Max_{JD}^{stored}$ and detects the malicious updates based on two empirically derived properties (or patterns). The first property that this algorithm employs to detect malicious updates from a client is to verify if its maximum Jensen-Divergence value is greater than some threshold factor. In this case, we empirically use an average of $Max_{JD}^{i}$ values stored in $Max_{JD}^{stored}$ (as observable in Figures~\ref{fig:cifar_iid}, \ref{fig:cifar_pmr}, and \ref{fig:WP_pmr}). The second property employed by this algorithm is the similarity of the maximum Jensen-Divergence values. In this case, we simply check if any $Max_{JD}^{i}$ is already present in $Max_{JD}^{stored}$, if yes, then we don't add the malicious update corresponding to the examined $Max_{JD}^{stored}$.
%\commentP{Can you clarify this here in 1 more sentence, analogously to the threshold for (i)?} 
(as observable in Figure~\ref{fig:iot_pmr}). The following addition has been made to \sect\ref{subsec:modules_design} (Filtering and Aggregation) and \sect\ref{subsec:algorithms} (\ourname WorkFlow and Algorithms) of the manuscript:}
\\
\answer{Filtering and Aggregation: }\changed{We encountered two patterns of malicious updates $Max_{JD}^{i}$ in our experiments, as discussed later in \sect\ref{sec:results}: (i) the $Max^i_{JD}$ computed for malicious updates was much greater than that for the benign updates, and (ii) the computed $Max^i_{JD}$ values for the malicious updates were similar. For pattern (i), we observed that the $Max_{JD}^{i}$ value for benign updates is less than the average of all the clients' $Max_{JD}^{i}$ values (experimentally evaluated). Therefore, conditioned on this observation, we filtered the malicious updates during the detection phase of \ourname. For pattern (ii), we check if $Max_{JD}^{i}$ of the incoming update is already present in the set of computed $Max_{JD}^{i}$ for the $n$ clients; if yes, we do not include the concerned malicious client's update in the final aggregation of updates to output the global model $G^{t}$.}
\\
\answer{\ourname WorkFlow and Algorithms: }\changed{
\ourname's workflow and detection algorithm have been outlined in Algorithms~\ref{algo:jensen} and \ref{algo:detection}. Here, $\mu_{0}$ is the assumed initial mean of the clusters and  $\sigma_{0}^{2}$ is the assumed variance corresponding to mean $\mu_{0}$. $\sigma_{w_i^t}^{2}$ is the measurement error of the client update $W_{i}^{t}$ and is computed as shown in Eq.~\eqref{eqn:3}. Thus, total measurement error or the variance is computed as shown in Eq.~\eqref{eqn:7}. If a new cluster is formed, it will have a normal distribution with mean $\mu_{0}$ and the combined variance of $\sigma_{0}^{2}$ + $\sigma_{w_i^t}^{2}$. The set $\{\mu_{c_{l}}^{t}$, $\sigma_{c_{l}}^{t}\}$ represents the mean and standard deviations of the $c_{l}$ clusters at time t.
%are \textbf{\textit{c_{l}}} clusters mean and standard deviation at time $t$.
We start Alg.~\ref{algo:jensen} by looping through the number of rounds of FL training as shown in line $2$. In each round, we initialize an empty array, $Max_{JD}^{stored}=[]$, to store the $Max_{JD}^{i}$ values of the clients. $n$ clients are selected for the training, and we loop through each client $i$ (line $4$) to determine its cluster. We then compute $W_{i, up}^{t}$ and $\sigma_{w_i^t}$ according to equations \eqref{eqn:2} and \eqref{eqn:3}, respectively (lines $7$). If $noc=0$, then it's the first round, and the first client is assigned to the first cluster (line $9$), and accordingly, this new cluster's $\mu_{new}$ and $\sigma_{new}$ are updated (line $10$). If $noc \neq 0$, then for each existing cluster plus the new one (line $12$), we do the following: first, we compute $p$ and $q$ (line $13$), second, we compute the \jensenDivergenceShort of each client's $p$ and each cluster's $q$ (line $14$), and third, we compute the maximum of the obtained \jensenDivergenceShort set ($Max_{JD}^{i}$) and decide the assigned cluster (line $15$) according to this value, and append it to the array $Max_{JD}^{stored}$ (line $16$). Either the client will be assigned to one of the already formed clusters (line $17$) or it will be assigned to a new cluster (lines $20, 21$). After each FL round, Algorithm \ref{algo:detection} ($DetectFilter()$) is called which takes input $Max_{JD}^{stored}$ (line $25$) and returns the filtered client updates, \textbf{\textit{fcp}}. $FedAVG(\textbf{\textit{fcp}})$ (defined in Appendix~\ref{app:fl}) algorithm is then performed to aggregate the filtered client updates and finally update the global model. 
}\\

\begin{algorithm}[tb]
\caption{\ourname's workflow.}
\label{algo:jensen}

\scalebox{0.9}{
\begin{minipage}{1.12\columnwidth}
\begin{algorithmic}[1]
\STATE \textbf{Input:} $\mu_{0}$, $\sigma_{0}^{2}$, $\sigma_{w_i^t}^{2}$, $\tau_{0} = \frac{1}{\sigma_{0}^{2}}$, $\tau_{w}=\frac{1}{\sigma_{w_i^t}^{2}}$, $noc$. 
%\STATE \textbf{Output:} Simulated values of the \textbf{\textit{c}} (clusters).
\FOR{ each round till the model converges }
    \STATE Initialize an array to store $Max_{JD}^{i}$ in each round, $Max_{JD}^{stored}=[]$.
    \FOR{ \textit{i} 1 $\leftarrow$ \textbf{to} n }
        \STATE Draw any client update $W_{i}^{t}$.
        \STATE Compute $d_{w_i^t}$ and $cos(W_{i}^{t},G^{t-1})$ . 
        \STATE Update $\sigma_{w_i^t}^{2}$ $\leftarrow$ $d_{w_i^t} \cdot cos(W_{t,i},G^{t-1})$ and compute $W_{i,up}^{t}$.
        \IF{$noc$ == 0}
        \STATE Assign $\textit{c}_{0} \leftarrow W_{i}^{t}$. 
        \STATE Update $\mu_{new}$ and $\sigma_{new}$ with, $n_{k}=1$. 
        \ENDIF
        \FOR{ \textit{$c_{l}$} $\leftarrow$ \textbf{to} \textit{noc+1}}
        \STATE Compute $p$ and $q$. 
        \STATE Compute the \jensenDivergenceShort by $p$ and $q$ and store the values.
        \STATE Decide the cluster, $c_{i}$ according to $Max_{JD}^{i}$.
        \STATE Append $Max_{JD}^{i}$ to $Max_{JD}^{stored}$.
        \IF{ $\textit{c}_{l,i}=c_{l}$}
        \STATE Update $W_{i}^{t}$ assigned cluster, $\{\mu_{c_{l}}^{t}$, $\sigma_{c_{l}}^{t}\}$ according to  $\textit{c}_{l,i}=c_{l}$.
        \ELSE 
        \STATE Increment $noc+1$, a new cluster is formed.
        \STATE Set $\textit{c}_{l,i}=noc$ and assign $W_{i}^{t}$ to it. Append this new cluster to the vector of non-empty clusters.
        \ENDIF
        \ENDFOR
    \ENDFOR
    \STATE Call $DetectFilter()$, \textbf{\textit{fcp}} = $DetectFilter(Max_{JD}^{stored})$. 
    \STATE Perform $FedAVG(\textbf{\textit{fcp}})$ and update the global model.
\ENDFOR
%\STATE \textbf{Return} $\textbf{\textit{c}}$.
\end{algorithmic}
\end{minipage}}
\end{algorithm}


\begin{algorithm}[tb]
\caption{Detection and Filter Algorithm, $DetectFilter$.}
\label{algo:detection1}

\scalebox{0.9}{
\begin{minipage}{1.12\columnwidth}
\begin{algorithmic}[1]
\STATE \textbf{Input: $Max_{JD}^{stored}$ containing $Max_{JD}^{i}$ values, total clients, $n$}
\STATE \textbf{Output: Filtered client updates}
    \STATE Initialize an array to store filtered client updates in each round, $W_{filtered}=[ ]$.
    \STATE Compute $Max_{JD}^{avg}$ = sum($Max_{JD}^{stored}$)/$n$
    \FOR{$ \mbox{i}=1 \mbox{ to } n$}
        \IF{$Max_{JD}^{i}$ not in $Max_{JD}^{stored}$ }
            \STATE $W_{filtered}$.append($W_{i}^{t}$)
        \ENDIF
        \IF{ $Max_{JD}^{i} < Max_{JD}^{avg}$}
            \STATE $W_{filtered}$.append($W_{i}^{t}$)
        \ENDIF
    \ENDFOR
\STATE \textbf{Return $W_{filtered}$} 
\end{algorithmic}
\end{minipage}}
\end{algorithm}




\textbf{R4.} Retract any claim of independence unless proven.\\
\answer{We reformulated the claims in the paper, %\commentAS{ Do not write you toned down, write your reformulated the claims in the paper}
 as described in R1.} \\
 
\textbf{R5.} Define "decoupled" as the authors do in the rebuttal; and add a note to say that in fact decoupling does not imply independence. \\
\answer{We explained what we meant by "decouple" in R1.}
%Decoupling refers to disassociating the functioning of the detection or clustering algorithm from any local client's training strategy as it does not administer the client's weights directly. 
%Also, we meant decoupling %\commentAS{You must first write what decoupling means. You are using the term decouple to explain decoupling, write first exactly what you mean by it, and then use the term decouple}
%the local client training from the defense mechanism, specifically in the detection part of the defense mechanism. 
%We use baseline BP to compute HBP for each client in a training round. In the first step of the \ourname, we assumed that the client weight vector ($W_{i, l}$) denotes the $l$ independent Bernoulli Process (BeP) draws over the likelihood function $A_{i, h}$ as mentioned in Section 2. $A_{i, h}$ is determined by its parameters, called the ''base measure'' and ''concentration function'', that we update in each training round given the new client updates. This step doesn't decouple the defense mechanism (as described above) as we use the client weights to update $A_{i, h}$ parameters or compute the posteriors. The motivation here is to leverage these parameters in the next step to decouple the detection part of the defense from the clients’ training, data distribution, and the number of clients selected in a training round. Hence, \ourname is not completely decoupled from the above factors, just the detection algorithm. Also, "decoupling" does not imply independence in our work. We have clarified this in Section~\ref{sec:introduction} (page 15) of the paper, as outlined below:}\\
%\changed{The first challenge is, how to compute an alternate representation of the client weights (probabilistic measure) that will represent the deviations made in the client weights and thus can be effectively used to decouple the detection/clustering part of the defense, i.e., detection of the malicious updates from any operations transpired on the client, such as adversarial training, different data distributions, or the number of clients selected in a training round. Here, decoupling refers to disassociating the functioning of the detection or clustering algorithm from any local client's training strategy as it does not administer the client's weights directly.} \\

\textbf{R6.} Expand the discussion of security guarantees provided by decoupling; in particular, the authors are encouraged to consider an adaptive attacker able to produce malicious updates by taking the BNP-inspired sampling procedure into consideration. \\
\answer{If we consider an adaptive adversary, who has the knowledge of the workings of \ourname, then the adaptive can only have access to base measure $H^{t}$, that can be updated given the current client's weights. This is because we are computing \jensenDivergence of the two distributions $p$ and $q$. $p$ is the distribution of the corresponding client that takes one of the inputs as base measure $H^{t}$ and can be computed by an adversary at runtime. However, since $q$ is the distribution of the clusters (existing clusters plus the new cluster), an adversary cannot estimate it as this requires knowing parameters that the server calculates on run-time. Thus, an adaptive attacker can only work with $H^{t}$ to launch backdoor attacks against such defense. We also conducted experiments with such an adaptive adversary and proved that \ourname effectively detects and filters adaptive adversaries updates. The results are shown in \sect\ref{subsec:strategies} (Adaptive attacks), as outlined below. We also expanded the discussion of security analysis against such an adaptive attacker in \sect\ref{sec:security} (Security Analysis), as clarified below:}\\
\answer{Adaptive attacks: } \changed{\ourname assumes that \adversary knows the backdoor defense deployed at the global server (cf.~\sect\ref{sec:threat}). Thus, \adversary can constrain the training process to make $H^{t}$ inconspicuous, by
%, which can be updated given the current client weights. 
%The reason is \adversary can 
using its benign data to estimate a benign model and, thus, $p$ and $H^t$. However, \adversary cannot estimate $q$ as this requires knowing parameters that the server calculates on run-time. Thus, an adaptive attacker can only work with $H^{t}$ to launch backdoor attacks against such defense. In this setting, we conducted experiments for the CIFAR-10,
%with such an adaptive adversary. Specifically, we 
by updating the loss function of \adversary using the base measure for the anomaly evasion loss term~\cite{bagdasaryan} according to the equation:  
\begin{equation}
    \mathcal{L} = \alpha \mathcal{L_{\text{class}}} + (1-\alpha) \mathcal{L_{\text{BM}}} \nonumber
\end{equation}
$\mathcal{L_{\text{class}}}$ captures both the BA and the MA, and $\mathcal{L_{\text{BM}}}$ captures the defense mechanism dependency on the base measure. We conducted three experiments with $\alpha$ (determines the trade-off between model accuracy and evasion from defense mechanism) values as 0.0, 0.5, and 1.0. For $\alpha=0.0$, \adversary sacrifices the model accuracy to evade the defense mechanism, for $\alpha=0.5$, \adversary is equally trading off the model accuracy and the defense mechanism evasion, and for $\alpha=1$, \adversary is more concerned about the model accuracy, than evading the defense mechanism detection.
For $\alpha=1$, \ourname was effective in detecting and filtering adaptive attackers model updates; achieved a $BA=0\%$, $MA =92.16\%$, and $TPR=1$. However, as we decreased the $\alpha$ to 0.5 and 0, $TPR$ reduced. For $\alpha=0.5$, \ourname obtained $BA=0\%$, $MA =92.16\%$, and $TPR=0.86$ ($TP=6$ and $FP=1$), and for $\alpha=0$, \ourname obtained $BA=0\%$, $MA =92.14\%$, and $TPR=0.36$ ($TP=4$ and $FP=7$). Hence, an adaptive adversary can evade the detection at the cost of model accuracy. However, the non-detected models do not have any overall impact on the efficacy of \ourname as the $BA$ is computed to be zero. In summary, our experiments show that \ourname is successful in defending against an adaptive adversary, with working knowledge of \ourname deployed at the global server
}\\
\answer{Security Analysis: }\changed{This section provides a security analysis to corroborate that \ourname can neutralize backdoors by modeling the defense mechanism using BNP modeling concepts. We explain why our defense works and justify its effectiveness.
To bypass our defense, an adversarial client (\adversary) has to ensure that \ourname cannot distinguish between malicious and benign model updates. Below, we present three mechanisms through which \adversary can hide the backdoors from \ourname. First, \adversary can vary the fraction (PMR) of malicious clients, i.e., \adversary can either reduce the PMR and make the attack less suspicious, or increase the PMR to keep the attack successful while making the models less suspicious. Second, \adversary can limit the poison data rate (PDR) for each of the adversarial clients, i.e., instead of poisoning the entire dataset, \adversary could partially poison the dataset. %However, this reduces the impact of the attack and makes it harder for \adversary.
Finally, \adversary can utilize an adaptive attack strategy, such as adding regularization terms (i.e., defense evasion) to the objective function of the training process (cf.\sect\ref{subsec:strategies}). A sophisticated \adversary with the working knowledge of \ourname (has access to the previous round base measure, $H^{t-1}$), could select a sweet spot between the model accuracy and the evasion from \ourname. As a result, the poisoned models are still similar to the benign models.

In all the above cases, we have demonstrated that \ourname successfully detected all the malicious updates. This is because \ourname computes an alternate, more generic representation of the client updates, i.e., a probabilistic measure that encompasses all the adjustments made to the client updates due to any local client's training strategy. Hence, the detection module that takes this probabilistic measure as one of its inputs correctly identifies all the malicious updates, without being affected by any local client training strategies. In addition, we also integrate the effect of $cos(W_{i}^{t},G^{t-1})$ and \lnorm (Eq.~\ref{eqn:2} and Eq.~\ref{eqn:3}) in the clients' model updates  and in the computation of error introduced by the client weight. The rationale is even though \adversary makes sure the distribution of malicious updates doesn't deviate from benign ones, \adversary cannot fully manipulate the $cos(W_{i}^{t},G^{t-1})$ or \lnorm, as \adversary's aim is to stimulate the global model in the backdoor direction. This ensures that any changes the strategic \adversary makes utilizing advanced hiding techniques cannot bypass \ourname. 
%\commentA{Why? you need to reason more detailed}
We also empirically verified the effectiveness of \ourname using \sota (CIFAR-10, MNIST, and FMNIST) and real-world (IoT) datasets and successfully demonstrated that \adversary cannot conduct backdoor attacks while simultaneously bypassing our defense mechanism. Therefore, \ourname is robust and resilient against backdoor attacks.} \\
    
% \commentAS{In the above text write always where in paper you have conducted all these actions. Always be precise}

\textbf{R7.} A better theoretical explanation or more convincing experimental analysis to support the use of BNP for detection (i.e. to demonstrate the differentiating capability). This could take the form of intuition for why the detection approach is good for backdoor detection. Ideally, this intuition should be supported by heuristic evaluation. \\
\answer{The \jensenDivergence (\jensenDivergenceShort) is used as a metric to identify malicious updates and assign them to new clusters: We define two distributions to compute \jensenDivergenceShort, $p$ distribution (related to clients) and $q$ distribution (related to clusters) in Section~\ref{subsec:modules_design} (mentioned below as well). Our experimental results (for the CIFAR-10, Reddit, MNIST, FMNIST, and IoT dataset) show that, for malicious updates, values in $p$ are either equal or close to zero. For benign updates, $p$ values lie at a larger distance compared to the malicious updates $p$ values (as the values in $p$ are either equal to or very close to zero), as shown in Figure~\ref{fig:JSD21} in this document. Thus, the distance between the malicious updates' $p$ values and the cluster's $q$ values is greater than the distance between the benign updates' $p$ and clusters' $q$ values. In other words, \jensenDivergenceShort($p$ (malicious updates), $q$) $>$ \jensenDivergenceShort($p$ (benign updates), $q$). Hence, maximum \jensenDivergenceShort is used as a metric to identify malicious updates and assign them to the new cluster.

%For the new cluster, we put mean=0 and std=1 and observed that the distance between the malicious updates' $p$ values and the new cluster's $q$ values is greater than the distance between the malicious updates' $p$ and existing clusters' $q$ values as shown in Figure~\ref{fig:JSD3} in this document.  In consequence, the \jensenDivergence($p$, $q$ (new cluster)) $>$ \jensenDivergence($p$, $q$ (existing clusters)). Thus, maximum \jensenDivergence, which is \jensenDivergence($p$, $q$ (new cluster)), was used to detect and assign malicious updates to the new clusters. 

$$p = \mathcal{N}(W_{i, up}^{t}; \mu_{p}, \sigma_{p})$$
$$p = x + H^{t-1} \quad \forall x \in p$$
\begin{equation}
    p = \mathcal{N}(p; 1, \overline{W_{i, up}^{t}}) \nonumber
\end{equation}

\begin{equation}
    q = \mathcal{N}(W_{i,up}^{t}; \mu_{c_{l}}, \sigma_{c_{l}}) \nonumber
\end{equation}

where, $\overline{W_{i, up}^{t}}$ is the mean of $W_{i,up}^{t}$ (updated client's update) and $\mu_{p}$ and $\sigma_{p}$ are the mean and the variance of the initial global model, respectively. $H^{t-1}$ is the round $t-1$ base measure that is given as $\frac{c_{i}^{t-1}}{c_{i}^{t-1}+l} H + \frac{1}{c_{i}^{t-1} \cdot l} \sum_{i = 1}^{l}W_{i}^{t-1}$ (cf. Eq.~\eqref{eqn:1}). $\mu_{c_{l}}$ and $\sigma_{c_{l}}$ are the clusters' mean and variance, respectively. This has been clarified in \sect\ref{sec:rationale} (Design: Intuition), as outlined below:}\\
\changed{To understand the relationship between the computed maximum \jensenDivergenceShort values $Max^i_{JD}$ (as outlined above) and the benign/malicious nature of the updates, we conduct experiments utilizing a diverse set of datasets (cf. \sect\ref{sec:setup}). In these experiments, we illustrated the $Max^i_{JD}$ values for malicious and benign updates and observed that $Max^i_{JD}$ values of malicious and benign updates differ significantly. Fig.~\ref{fig:JSD3} gives an intuition of why $Max^i_{JD}$ differs for the malicious and benign updates by examining the range of $p$ distribution values for the client updates against the clusters' $q$ distribution values. In Fig.~\ref{fig:JSD3}, the (i) plot demonstrates the malicious update's $p$ values spanning area, the (ii) plot demonstrates the benign update's $p$ values spanning area, and the (iii) plot demonstrates the clusters' $q$ values spanning area, as observed from the experiments conducted. As seen in these plots, the benign update's $p$ values lie at a larger distance than the malicious update's $p$ values (as the values in $p$ are either equal to or very close to zero). Thus, the distance between the $p$ values of malicious updates, and the  $q$ values of the clusters is greater than the distance between the  $p$ and $q$ values of benign updates. In other words, \jensenDivergenceShort($p$ (malicious update), $q$) $>$ 
\jensenDivergenceShort($p$ (benign update), $q$). Hence, maximum \jensenDivergenceShort is used as a metric to identify malicious updates and assign them to the new cluster.
}


%clients' $p$ distribution is computed as: $N(p;1,W_{i,l}^{up})$ and clusters' $q$ distribution is computed as: $N(W_{i,l}^{up};\mu_{c}, \sigma_{c})$. $W_{i,l}^{up}$ is the update

%For the new cluster, we put $\mu_c = 0$ and $\sigma_c = 1$ and observed that for malicious updates, values in $p$ are either equal to or very close to zero (from CIFAR-10, Reddit, MNIST, FMNIST, and IoT dataset experiments), shown in Figure~\ref{fig:JSD3}. From these experiments, it can be observed that a new cluster's $q$ distribution distance from the origin is greater than the distance of the existing clusters' $q$ distribution from the origin. In other words, \jensenDivergence($p$, $q$ (new cluster)) $>$ \jensenDivergence($p$, $q$ (existing clusters)). Hence, maximum \jensenDivergence is used as a metric to identify malicious updates and assign them to the new cluster. }\\

\begin{figure}[!ht]
\centering
\includegraphics[width=3.5in]{figures/JD3.png}
\caption{$p$ and $q$ distribution value range for the malicious updates, benign updates and the clusters': (i) the malicious updates $p$ values spanning area, (ii) the benign updates $p$ values spanning area, and (iii) the clusters' $q$ values spanning area, as observed from the experiments conducted for five datasets.}
\label{fig:JSD3}
\end{figure}

\textbf{R8.} Add clear and consistent detection criteria (in section 5, the detection part). The authors observed two different cases in the experiments in Section 6: a) malicious clients have larger JD, and b) malicious clients have similar JD but exhibit lower variance. The paper would be stronger if a consistent detection rule could be identified and evaluated across multiple datasets. \\
\answer{We have outlined in detail a consistent detection algorithm, as discussed in the response R3 above. Moreover, we have also conducted additional experiments for the MNIST (App.~\ref{app:mnist}) and FMNIST (App.~\ref{app:fmnist}) datasets to prove the efficacy of the proposed \ourname malicious update detection framework. Due to space constraints, we have moved the experimental results of FMNIST and MNIST to Appendix. We evaluate the impact of \nonIid rate and $PMR$ on both MNIST and FMNIST datasets. To estimate the impact of different \nonIid values, we set $PMR=0.2$; the default $PMR$ value for Image classification applications. Similarly, to estimate the impact of different $PMR$ values, we set \nonIid = 0.7; the default \nonIid value for Image classification applications. Please refer to Figures~\ref{fig:fmnist_iid} and \ref{fig:fmnist_pmr} for the experimental results of the FMNIST dataset and Figures~\ref{fig:mnist_iid} and \ref{fig:mnist_pmr} for the experimental results of the MNIST dataset in the Appendix.}\\
\answer{FMNIST: }\changed{In this section, we evaluate the impact of \nonIid rate and $PMR$ on the FMNIST dataset. First, we demonstrate the trend of $Max_{JD}^{i}$ for both the malicious and benign clients, with respect to each of these parameters. Then, we illustrate the impact of \nonIid rate and $PMR$ on \ourname's performance by quantifying different metrics as stated in \sect\ref{sec:setup} and also compare it against the no defense scenario. 

\noindent
\textbf{Illustration of $Max_{JD}^{i}$. }
Impact of the degree of \nonIid data and $PMR$ on $Max_{JD}^{i}$ for each client is shown in Fig.~\ref{fig:fmnist_iid} and Fig.~\ref{fig:fmnist_pmr}, respectively. We select a total of 30 (\numberOfClients = 30) clients for both the \nonIid and $PMR$ experimental analysis. For \nonIid analysis, we test \nonIid $\in \{0.0, 0.5, 1.0\}$ and set $PMR=0.2$. Thus, number of malicious clients equals 6 (\numberOfMaliciousClients = 6). For $PMR$ analysis, we test $PMR \in \{0.2, 0.3, 0.5\}$, i.e., when $\numberOfMaliciousClients$ equals 6, 9, and 15 and set \nonIid = 0.7. As illustrated in Fig.~\ref{fig:fmnist_iid} and Fig.~\ref{fig:fmnist_pmr}, the $Max_{JD}^{i}$ value for benign clients differs significantly from that of malicious clients. Hence, \ourname easily filters out all the malicious client updates, achieving a $BA$ of zero while keeping the $MA$ of the global model intact.
}\\
\answer{MNIST: }\changed{
 In this section, we evaluate the impact of \nonIid rate and $PMR$ on the MNIST dataset. First, we demonstrate the trend of $Max_{JD}^{i}$ for both the malicious and benign clients, with respect to each of these parameters. Then, we illustrate the impact of \nonIid rate and $PMR$ on \ourname's performance by quantifying different metrics as stated in \sect\ref{sec:setup} and also compare it against the no defense scenario. 

\noindent
\textbf{Illustration of $Max_{JD}^{i}$. }
Impact of the degree of \nonIid data and $PMR$ on $Max_{JD}^{i}$ for each client is shown in Fig.~\ref{fig:mnist_iid} and Fig.~\ref{fig:mnist_pmr}, respectively. We select a total of 30 (\numberOfClients = 30) clients for both the \nonIid and $PMR$ experimental analysis. For \nonIid analysis, we test \nonIid $\in \{0.0, 0.5, 1.0\}$ and set $PMR=0.2$. Thus, number of malicious clients equals 6 (\numberOfMaliciousClients = 6). For $PMR$ analysis, we test $PMR \in \{0.2, 0.3, 0.5\}$, i.e., when $\numberOfMaliciousClients$ equals 6, 9, and 15 and set \nonIid = 0.7. As illustrated in Fig.~\ref{fig:mnist_iid} and Fig.~\ref{fig:mnist_pmr}, the $Max_{JD}^{i}$ value for benign clients differs significantly from that of malicious clients. Hence, \ourname easily filters out all the malicious client updates, achieving a $BA$ of zero while keeping the $MA$ of the global model intact.
}\\

\textbf{R9.} Incorporate the changes discussed in the rebuttal submitted by the authors. \\
\textit{Dataset descriptions.} \answer{The NIDS and WP applications both use sequences of symbols, representing network packets in the NIDS application and words in the WP application, to predict the next symbol. Aligned with the work of Bagdasaryan~\etal \cite{bagdasaryan}, we focus on the WP application on the \numprint{50000} most frequent words as symbols, resulting in \numprint{50000} output classes. For the NIDS application, we generated 695 different symbols. As stated in the \diot paper \cite{nguyen2019diot}, the NIDS dataset is already publicly available. For our evaluation, we instantiated the \diot system as real-world application. Therefore, we replaced \fedavg by \ourname but did not change the remaining \diot system. We used the exact NN architecture and training procedure as defined by Nguyen \etal  in the \diot paper \cite{nguyen2019diot}, which is a recurrent neural network, consisting of 2 layers with Gated-Recurrent-Units (GRU), followed by a fully connected linear layer. We clarified this in \sect\ref{sec:setup} (Experimental Setup).}\\
\changed{\emph{Word Prediction (WP):} To evaluate \ourname for a complex Natural Language Processing (NLP) application such as word prediction, we use the Reddit dataset consisting of all posts from November 2017. Aligned with the work of Bagdasaryan~\etal, we considered each author's posts as a local dataset and only the 50K most frequent words. A Long Short-term Memory (LSTM) model is used to predict the next word~\cite{bagdasaryan}.}\\
\changed{\emph{Network Intrusion Detection (NIDS):} Further, we evaluate \ourname for the FL-based NIDS \diot~\cite{nguyen2019diot} system using four real-world network traffic datasets, kindly shared with us by Nguyen~\etal~\cite{nguyen2019diot,nguyen22Flame} and Sivanathan~\etal~\cite{sivanathan2018UNSWdata}. The datasets consist of network traffic of multiple smart home and office settings. Aligned with previous work~\cite{nguyen22Flame,rieger2022deepsight}, we converted the network packets into symbols based on their features, such as source and destination port, protocols, and flags. To simulate a distributed FL setting, the dataset was split into 100 local datasets, each consisting of between 2K and 3K symbols which were extracted from the network packets. The NN is trained to predict the next probabilities for each possible symbol (network packet). The NN consists of 2 Gated-Recurrent-Unit layers followed by a fully connected linear layer, as defined by Nguyen~\etal~\cite{nguyen2019diot}.}


\emph{Extend Evaluation}\\
\answer{The discussed experiments are provided as part of Major Revision requirement R6 and Major Revision requirement R8.}

\emph{Adapt background section}\\
\answer{We adapted the background section (\sect\ref{sec:background}) and adjusted the text as following:}\\
\changed{
Our approach is modeled in two steps. First, to determine the probabilistic distributions of clients' updates, we make use of several statistical tools such as Beta Processes (BP), Hierarchical Beta Processes (HBP), and Bernoulli Processes (BeP).
%, represented by the posterior of the HBP parameters given the new client updates. 
Second, to design our detection algorithm, we design an adaptation of the Chinese Restaurant Process (CRP), called CRP-Jensen, to detect and filter out malicious updates. Below, we briefly discuss the above two steps (see more technical details in the Appendix):
%\begin{enumerate}[leftmargin=*]
    %\item 
\noindent\\
\textbf{Determining probabilistic measure for client updates.} We compute the probabilistic measure for each client selected in an FL round to keep track of the adjustments made during each update. For this, we first draw a baseline probabilistic measure, denoted by the baseline Beta Process (BP), which is computed using the initial global model. Informally, a BP is a process quantifying a subset of points (measure). We use BPs in this work to quantify the client updates and the global model by creating distributions over them.
%, and we use it here to quantify the client updates and the global model. In this work, we quantify the client updates and the global model by creating distributions over them.
    
A BP ($A$) is a stochastic process defined using two parameters: a concentration function $c$ over some space $\Omega = \mathbb{R}$ and a base measure $H$; denoted as $A \sim BP(c, H)$. In the FL context, the base measure $H$ can represent any distribution of the initial global model (cf.~\sect\ref{sec:rationale}), i.e., before the training starts, and a concentration function $c$ quantitatively characterizes the similarity between the input base measure ($H$) and the output random measure $A$ (because of the distribution over the random selection of elements in $\Omega$). In this work, $c$ determines the similarity between the input and the output distribution over $\Omega$, and $\Omega$ is a collection of initial global model weights. The intuition here is to first use this baseline BP, called baseline BP \emph{prior}, to form hierarchies of BP, called hierarchical BP prior, for $n$ different clients selected in the first FL round, i.e., create $n$ sub-BP from the baseline BP. In other words, create $n$ sub-distributions over $\Omega$ from the baseline distribution over $\Omega$.
    %In other words, the parameters of the HBP, i.e., $c_{i}$ and $H_{i}$, will keep updating the subsequent iterations of the FL, given the new client updates.

    
Informally, a \emph{prior} is the previous knowledge of an event before any new empirical data is observed and is typically expressed as a probability distribution or random measure, while a \emph{posterior} is the revised or updated knowledge of the event after considering the new data. Now, a HBP for each client $i$ is denoted as $A_{i} \sim BP(c_{i}, A$). In the subsequent iterations of the FL, these priors (as computed above) will be updated, based on the new client updates, to compute the so-called BP posteriors, i.e., update the $c_{i}$ and $H_{i}$ ($A_{i}$). In this work, we have assumed the new client updates in each round as the new data to update the previous knowledge of the BP priors, i.e., to compute the BP posteriors.
    
In this work, we flatten updates for each client $i$ to a one-dimensional vector having $l$ values, denoted as $W_{i}$. We assume that each value in this vector is drawn from a Bernoulli Process (BeP), given the client $i$'s BP random measure $A_{i}$. Informally, a BeP is a stochastic process with two possible outcomes: success or failure $-$ we use it in this work to show whether a client $i$'s update will have a particular value or not, given its BP random measure $A_{i}$. In FL, each client updates its local model using the common aggregated global model sent by the global server. Hence, we postulate that each client update vector values are drawn from its corresponding BP random measure $A_{i}$, using BeP. Thus, a weight vector $W_{i}$ for client $i \in \{1,...,n\}$ is characterized by a Bernoulli Process, given as $W_{i} | A_{i} \sim \text{BeP}(A_{i})$. In other words, in $W_{i} = \{W_{i,1}, W_{i,2}, ..., W_{i,l}\}$, $l$ denotes the independent BeP draws over the likelihood function $A_{i}$.

Another reason to use BeP is that it has been shown in the literature that the Beta distribution is the conjugate of the Bernoulli distribution~\cite{broderick2018posteriors}. Hence, we do not have to use the computationally intensive Bayes' rule to compute the posteriors. Hence, we keep updating the corresponding HBP ($A_{i}$) for client $i$ using the conjugacy of the BP and the BeP, as given in \cite{thibaux2007hierarchical}. The posterior distribution of $A_{i}$ after observing $W_{i}$ is still a BP with modified parameters:
    \begin{equation}
        A_{i}|W_{i} \sim BeP\left(c_{i}+l, \frac{c_{i}}{c_{i}+l} H + \frac{1}{c_{i} \cdot l} \sum_{l = 1}^{l}W_{i} \right) \nonumber
    \end{equation}

%\item 

\noindent\textbf{Designing the backdoor detection algorithm.} Next, we briefly describe how we adapt the Chinese Restaurant Process to detect malicious client updates. The CRP~\cite{socher2011spectral,blei2011distance,li2019tutorial} is an infinite (unknown number of clusters) mixture model in which customers (client's updates) are assigned tables (clusters) in a restaurant. In the context of FL, the clusters represent groups of incoming client updates. The customer can either sit at the already occupied tables (existing clusters) or at the new table (a new cluster is created). 
%\commentA{CRP computes the predictive probability to decide the assignment of a customer to an existing table or a new table.} 
Our main idea, as discussed earlier, is to utilize a probabilistic measure to determine the distribution of the incoming local client $i$'s update. We also compute the distribution of the existing clusters of updates plus the new cluster. Then, we compute the \jensenDivergence between client $i$'s update distribution and each existing plus new cluster's distribution. Informally, \jensenDivergence (or Jensen-Shannon Divergence) is a procedure to measure how two distributions are similar.
In consequence, we obtain a set of \jensenDivergence values. We take the maximum of this set to determine whether local client $i$ is malicious or not (intuition, as to why use maximum \jensenDivergence, is shown in \sect\ref{sec:rationale}). Based on this maximum \jensenDivergence value, we also determine the client $i$'s update cluster assignment. 
%of the two distributions to compute the fit of the client $i$ to an existing or a new cluster. 
After the cluster is determined, we append the client $i$'s update to the selected cluster's list of client updates. Finally, we update the cluster's parameters, i.e., mean and standard deviation, using \textit{Chinese Restaurant Process (CRP)}. This adaptation of the CRP is also referred to by us as CRP-Jensen. 

}

\emph{Symbol Table}
\answer{We have added a Table of symbols in the Appendix (Appendix~\ref{app:symbols}).
}



 
 
\section{RESPONSES TO INDIVIDUAL REVIEWS}

\subsection*{REVIEWER  A}

\textbf{A1.} The background section does not provide all the necessary information for the average reader.
What I would like to see is a bit more discussion about some statements and a comparison with~\cite{yurochkin2019bayesian}. \\
\answer{The main motivation in~\cite{yurochkin2019bayesian} is to reduce the communication overhead between the clients and the global server by reducing the number of training rounds. However, our objective in this paper is completely different and aims at effectively filtering out malicious updates. To achieve their goal, the authors in~\cite{yurochkin2019bayesian} used a Beta-Bernoulli Process (BBP) to optimize the selection of global atoms by finding the common subset of neurons between the local clients selected in a training round and combining them to form a global model. However, we use a Baseline BP to compute Hierarchical Beta Process (HBP) for the clients selected in the training round and leverage them in the detection phase to filter the malicious updates. This has been clarified in \sect\ref{sec:introduction} (Introduction).}
\\
\changed{There has been one related research effort~\cite{yurochkin2019bayesian} in the literature that has employed similar Bayesian non-parametric (BNP) models in the FL context~\cite{yurochkin2019bayesian}. In that work, the authors used BNP models, specifically the Beta-Bernoulli Process and the Indian Buffet Process, to reduce the communication overhead between the global server and the clients. They accomplished this by finding the common subset of neurons between the local clients selected in a training round and combining them to form a global model. In contrast to their work, we employ BNP models, specifically the Hierarchical Beta-Bernoulli process and CRP, to design a defense mechanism against backdoor attacks in FL. Also in \cite{yurochkin2019bayesian}, an adversary's training updates can easily be integrated into the global model as the authors are trying to optimize the selection of the global model updates. Thus, their work is vulnerable to backdoor attacks in FL.}\\


\textbf{A2.} Consequently, the defense mechanism remains agnostic about any attack methodology that an adversary can design. how can we be sure about this? Even if the attack uses info that BayBFed is used, no better attack can be made? \\
\answer{This comment was addressed by Major Revision requirement R6.}\\

\textbf{A3.} I would like to see a better discussion on those differences with~\cite{yurochkin2019bayesian}. What does it mean in practice? Would \cite{yurochkin2019bayesian} not provide a good defense?\\
\answer{Answered in A1. As~\cite{yurochkin2019bayesian} only performs an optimal matching of the client updates to find the optimal global atoms, an adversary’s training update can be inadvertently integrated into the global atoms computation, thus making the approach vulnerable to manipulation by individual clients.}\\

\textbf{A4.} In the experiments, we choose a random baseline of c = 5. why that value? From what range is it taken?\\
\answer{Initially, this value was chosen randomly. It did not affect the experimental results as we keep updating its value by computing the posterior given the new client updates. We have clarified this in \sect\ref{sec:rationale} (Design) as follows:}\\
\changed{In the experiments, we initially choose a random baseline of $c=5$ and continuously update it given the new client weights.}\\
%Copy from supplementary rebuttal

\textbf{A5.} Please explain why using the constraints-and-scale and Edge-case backdoor attacks. How does it cover the most important settings? \\
\answer{These attacks cover the most important attack strategies: data poisoning, projected gradient descent, and boosting the updates through scaling. To enable an equitable comparison, we aligned our experimental setup with the setups of other state-of-the-art papers focusing on backdoor attacks (e.g.,  \cite{andreina2020baffle,bagdasaryan,nguyen22Flame,shen16Auror,wang2020attack}), which also focus their evaluation on these strategies for backdoor injection. We clarified this in \sect\ref{sec:setup} (Experimental setup) as follows:}\\
\changed{Aligned with previous work on backdoor attacks~\cite{andreina2020baffle,bagdasaryan,nguyen22Flame}, we use the attacks provided by Bagdasaryan \etal~\cite{bagdasaryan} and Wang \etal~\cite{wang2020attack} to implement the \ConstrainAndScale and Edge-Case backdoor attacks.}\\

\textbf{A6.} The description of the datasets is uneven. Could the authors make the dataset publicly available or ask the authors of [27] [28] to do so?\\
\answer{This comment is addressed as part of major revision requirement R9.}\\

\textbf{A7.} Finally, I could not find any results for MNIST anywhere in the paper? \\
\answer{We performed an experiment for MNIST, achieving 43.0\% BA and 96.5\% MA without defense, while \ourname reduced the BA to 0.0\% and kept the MA at 96.0\%. We have added these results to Table ~\ref{tab:success_attacks} in \sect\ref{sec:results} (Experimental Results). Due to space constraints, we have moved MNIST dataset results to Appendix \ref{app:mnist}.} \\

\textbf{A8.} The authors say they use six defenses, but is it actually seven? \\
\answer{Yes, the reviewer is correct. We have fixed this oversight in \sect\ref{sec:results} (Experimental Results), as follows:}
\\
\changed{We compare \ourname against seven \sota defense mechanisms present in the literature: Krum~\cite{blanchard17Krum}, FoolsGold~\cite{fung2020FoolsGold}, Auror~\cite{shen16Auror}, AFA \cite{munoz19AFA}, DP~\cite{yin2018byzantine}, Median~\cite{mcmahan2017learning} and FLAME~\cite{nguyen22Flame}.}\\

\textbf{A9.} Please discuss why BayBFed increases MA for CIFAR-10 when using Constraints-and-scale?\\
\answer{\ourname does not increase the MA for CIFAR-10. As we can see in Table~\ref{tab:success_defenses} in Section~\ref{sec:results}, 92.6 is the MA for the benign setting. When the attack is performed, the MA is reduced to 90.5 if no defense setting is considered. Therefore, the attack (without the BayBFed defense) has the side effect of reducing the MA. When BayBFed is employed, the attack is mitigated, as well as this side effect. We have clarified this in \sect\ref{sec:results} (Experimental Results), as follows:}\\
%todoPhillip color something; refer section of table
\changed{For the IC application and in the case of the CIFAR-10 dataset, we observe that the \ConstrainAndScale attack lowers the MA from 92.6\% (FedAVG without attack) to 90.5\% (FedAVG). Krum, FoolsGold, Auror, DP, and Median techniques achieve a $MA$ of 56.7\%, 52.3\%, 26.1\%, 78.9\%, and 50.1\%, respectively, which is considerably lower than the benign setting $MA$. In contrast, \ourname has a $MA$ of 92.2\%, which shows that it works significantly better for IC applications.}\\

\textbf{A10.} I am a bit surprised with the results for BA, where we see all the numbers either 100\% or 0\% (except for DP). Why is that? \\
\answer{Each defense, which we have comparatively evaluated in this work, makes specific assumptions about the data and attack scenarios and is only effective under those assumptions but performs erroneously if the assumptions do not hold. For instance, in the case of Krum~\cite{blanchard17Krum}, which selects a single model as an aggregated model, a poisoned model is chosen when an attacker circumvents the Krum. Therefore the aggregated model is fully replaced by a poisoned model, achieving 100\% BA. Similarly, another defense FoolsGold [14], assumes that the benign models differ significantly from each other. As long as this assumption is satisfied, the defense remains effective against the evaluated attacks. However, when this assumption does not hold (for example, multiple benign clients submit similar models), FoolsGold fails to recognize the benign models and is ineffective against the evaluated attacks. We have clarified this in \sect\ref{sec:results} (Experimental Results), as follows:}
\\
\changed{Further, these defense mechanisms perform accurately when specific assumptions about the data and attack scenarios are satisfied. For instance, in the case of Krum~\cite{blanchard17Krum}, which selects a single model as an aggregated model, a poisoned model is chosen when an attacker circumvents Krum. Therefore, the aggregated model is entirely replaced by a poisoned model, achieving 100\% BA. Similarly, another defense FoolsGold~\cite{fung2020FoolsGold}, is effective for the highly \nonIid Reddit dataset but fails when their clients have similar data. }\\


\textbf{A11.} Why do Sections 7.2 and 7.3 consider 30 clients only? And 7.4 60? I am not saying the number is not OK, but please motivate.\\
\answer{We considered 30 clients for the Image classification application and 60 for the NIDS application because of the training time. FL training for Image classification takes longer than for the NIDS application. However, as we kept the PMR rate the same for both cases, we do not anticipate a significant impact of the different number of clients on the overall experimental results. We have clarified this in \sect\ref{subsec:iot} (Experimental Results), as follows:}\\
\changed{It should be noted that since NIDS models have lesser number of parameters, training time is reduced. Thus, we evaluated more clients than WP and IC models/applications. However, we set the same $PMR$ in all scenarios. Hence, it did not impact the experimental results (except for the experiments where we considered different $PMR$s).}\\
%\toDiscuss{Check how much to put to paper}
%todoPhillip

\textbf{A12.} We perform four experiments for the NIDS application, where each client is trained to inject 1 to 4 backdoors. -$>$ why up to 4? \\
\answer{We have clarified this in \sect\ref{sec:results} (Experimental Results), as follows:}\\
\changed{We perform four experiments for the NIDS application, where each client is trained to inject 1 to 4 backdoors. Existing work \cite{rieger2022deepsight} has shown that the attack efficiency significantly reduces as the number of backdoors increases, and we observed the same pattern during our experiments. Hence, four backdoors were considered a good number (of backdoors) that provided reasonable attack efficiency. Our evaluations show that \ourname was able to defend against and mitigate all the introduced backdoors effectively, thus achieving a 0\% BA. }\\
%\changed{We perform four experiments for the NIDS application, where each client is trained to inject 1 to 4 backdoors. However, \ourname always detects all poisoned models without having any FP, s.t., the BA remains $0\%$. In parallel, without defense, the effectiveness of the attack was decreased with an increasing number of backdoors.}\\
%Copy from supplementary rebuttal
%todoPhillip

\textbf{A13.} An adversary can launch backdoor attacks by either manipulating the weights or by poisoning the data. -$>$ After reading this sentence, I somehow expect to see results for code poisoning as well? \\
\answer{We have clarified this in \sect\ref{sec:results} (Experimental Results), as follows:}\\
\changed{The effectiveness of \ourname against two \sota model poisoning attacks, the \ConstrainAndScale~\cite{bagdasaryan} and the Edge-Case backdoor~\cite{wang2020attack} is shown in Tab.~\ref{tab:success_attacks}. In our threat model, we have considered a strong adversary that can perform arbitrary operations for the attack, including code poisoning attacks.
%including changing the code that trains the model. Thus, our considered attack scenarios also include attacks such as code poisoning attacks. 
As our adversary is assumed to fully control the malicious clients (and thus the code on the clients), he is not restricted or constrained in terms of the employed attack strategy. In addition to attacks during training, our adversary can also adopt a runtime strategy to make the attack more stealthy. }\\
%\changed{The effectiveness of \ourname against 2 \sota model poisoning Attacks, the \constrainAndScale~\cite{bagdasaryan} and the \textit{Edge-Case backdoor}~\cite{wang2020attack} is shown in Tab.~\ref{tab:success_attacks}. Compared to other attacks, e.g., data poisoning~\cite{shen16Auror,nguyen2020diss} or code poisoning~\cite{bagdasaryan2021blind}, in the considered model poisoning attacks \adversary does not have any restrictions but fully controls the malicious clients.}\\
%Theoretical justification in rebuttal document: Covered by Model Poisoning
%todoPhillip

\textbf{A14.} Algorithm 1 is not the full workflow? There is no removal of poisoned samples? \\
%Copy from supplementary rebuttal
\answer{We have answered this in R3.} \\

\textbf{A15.} Checking the results, we see that for one attack, BA is above 0\%, which means that the attack still could be possible? \\
\answer{In the case of images when a pixel-based trigger is used, the BA, even for a backdoor-free model, can be greater than 0\%. As already pointed out by Rieger~\etal, if models predict some images incorrectly (therefore, MA $<$ $100\%$), the model may also classify some images as the backdoor target label. However, when computing the BA, these wrong predictions are counted as backdoor affected predictions~\cite{rieger2022deepsight}. Therefore, the BA is above 0\% for some attacks. For example, in the case of edge-case backdoor attacks, where the initial BA, i.e., before the attack, is 11.22\%. \ourname mitigated the attack. We have clarified this in \sect\ref{sec:results} (Experimental Results), as follows:}\\
\changed{It should be noted that if the MA is less than 100\%, misclassifications of the model can be counted in favor of the backdoor, especially if the model wrongly predicts the backdoor target. As already pointed out by Rieger~\etal~\cite{rieger2022deepsight}, this phenomenon especially occurs for image scenarios with pixel-based triggers. It causes the BA to be slightly higher than 0\% for backdoor-free models. In the case of an Edge-Case attack, the BA before the attack is 11.22\% and 4.02\% after \ourname, while without defense, the BA achieves 33.16\%.}\\
% In our experiments, without the attack
%Therefore, 


\textbf{A16.} not clear why the authors consider only health cases and not more general ones? If the health case is the most important, why not give some experimental results for it? \\
\answer{Different applications have been developed that can benefit from FL. Besides health applications, other real-world applications of FL include, but are not limited to, Natural Language Processing for SmartpNetwork \cite{mcmahan2017googleGboard} and collaborative Network Intrusion Detection Systems (NIDS) for IoT devices \cite{nguyen2019diot}. To simplify the comparison we aligned our experimental setup with existing work~\cite{bagdasaryan,rieger2022deepsight} and focused on the NIDS and NLP applications. We have emphasized these applications in \sect\ref{sec:introduction} (Introduction) as follows:}\\
\changed{Learning a single machine learning model by using this scattered data is complex and challenging as it may disclose a user's identifiable and protected information. Federated Learning (FL) promises to significantly reduce the impact of such drawbacks by enabling multiple distributed clients to cooperatively learn a global server model~\cite{mcmahan2017,yang2018applied}. For instance, multiple hospitals can participate in training a global model for cancer classification without revealing individual patients' cancer records~\cite{li2020federated,sheller2018medical,xu2021federated}. Similarly, multiple smartphones could train together a word suggestion model without sharing the individually typed texts~\cite{mcmahan2017googleGboard}.}\\
%Additional experiment: malaria
%todoPhillip

\textbf{A17.} What makes CIFAR-10 a state-of-the-art benchmark dataset?\\ 
\answer{Both the CIFAR-10 and MNIST datasets have been frequently used not only for measuring the effectiveness of FL approaches~\cite{mcmahan2017,sattler2020clustered}, but also to evaluate backdoor attacks and defenses~\cite{bagdasaryan,cao2021provably,fung2020FoolsGold,guerraoui2018hidden,khazbak2020mlguard,li2020learning,munoz19AFA,nguyen22Flame,rieger2022deepsight,wang2020attack,wu2020mitigating,xie2021crfl}. Their wide usage in many prior publications allows a simplified comparison of the different approaches in the literature. We have clarified this in \sect\ref{sec:setup} (Experimental Setup), as follows:}\\
\changed{
We use the popular benchmark datasets MNIST, FMNIST, and CIFAR-10 in our experiments. As these datasets are frequently used for evaluating FL and backdoor attacks and defenses~\cite{bagdasaryan,cao2021provably,fung2020FoolsGold,guerraoui2018hidden,khazbak2020mlguard,li2020learning,mcmahan2017,munoz19AFA,nguyen22Flame,rieger2022deepsight,wang2020attack,wu2020mitigating,xie2021crfl}, it enables us to perform an equitable comparative analysis of our approach with other state-of-the-art approaches in the literature.
}

\subsection*{REVIEWER B}

\textbf{B1.} Can you clarify why/how the datasets are representative? \\
\answer{As mentioned in Section 6, the datasets that we use in our paper have been used in different attack settings in the literature ([3], [8], [23], [13], [28], and [26]). That is one of the main reasons we employ these datasets in the evaluation of \ourname. Another reason for using these datasets is that they are being used to train models in different application domains; for example, CIFAR10 has been used extensively in the healthcare industry \cite{xu2021federated,kim2018keep}, in human supervision \cite{arazo2020pseudo}, object detection \cite{mccann2013object}, etc. Reddit dataset has also been used in different applications such as stress analysis in social media \cite{turcan2019dreaddit}, demographics \cite{gjurkovic2020pandora}, etc. We have clarified this in \sect\ref{sec:setup} (Experimental Setup), as follows:}\\
\changed{To show the generality of our results and the representative nature of \ourname across models/data from different domains, we evaluate the proposed defense mechanism by designing two attacks (cf. in Tab.~\ref{tab:success_attacks}) on three popular FL applications: (i) image classification, (ii) word prediction, and (iii) IoT network intrusion detection. To facilitate an equitable comparison of \ourname with state-of-the-art backdoor attack approaches~\cite{bagdasaryan,nguyen22Flame}, we align the datasets, setups, and NN architectures employed in our comparative evaluation \mbox{with the ones used by these research efforts.}}\\

\textbf{B2.} Can you clarify the main takeaways and improvements over SOTA? \\
\answer{We introduced a Bayesian defense mechanism that leverages concepts from non-parametric Bayesian modeling to filter out malicious updates. It works in two phases: in the first phase, we compute Hierarchical Beta posteriors for each client given the client’s weight updates, and in the second phase, we use these Beta posteriors to make the defense independent of the local client training, attack strategy of the malicious clients, data distributions and number of the clients selected in a training round. This is an improvement over previous defense mechanisms as they work only when certain conditions are met. We have clarified this in \sect\ref{sec:conclusion} (Conclusion), as follows:}\\
\changed{
We presented \ourname, a novel and more generic probabilistic approach to defend against backdoor attacks in Federated Learning. 
In contrast to existing defenses that mainly consider models as a set of vectors and matrices~\cite{blanchard17Krum,fung2020FoolsGold,mcmahan2018iclrClipping,munoz19AFA,nguyen22Flame,shen16Auror} and operate \emph{directly} on them, \ourname first computes a probabilistic measure over the clients' updates that encompass all the adjustments made in the updates due to any local client training strategy. Then, \ourname employs a detection algorithm that utilizes this probabilistic measure to detect and filter out malicious updates. Thus, it overcomes the shortcomings of the previous approaches. \ourname utilizes two extensions of Bayesian non-parametric modeling techniques: the Hierarchical Beta-Bernoulli process to draw a probabilistic measure given the client’s model update (i.e.,weights), and a variation of Chinese Restaurant Process, CRP-Jensen, which is a clustering algorithm that can leverage the probabilistic measure to detect and filter out the malicious updates. Our extensive evaluation on datasets in different domains demonstrates that \ourname effectively can mitigate backdoor attacks in FL while preserving the \mbox{benign performance of the global model.}
}\\

%todoPhillip rephrase conclusion

\subsection*{REVIEWER  C}

\textbf{C1.} Why the maximum Jensen-Divergence can be used for filtering malicious models? \\
\answer{This comment has been addressed in our response to R7.}\\

\textbf{C2.} A detailed definition of Jensen-divergence is not provided. Do the authors refer to the Jesen-Shannon divergence? \\
\answer{Yes, when we mention \jensenDivergence in the paper, we mean Jensen-Shannon divergence. Due to space constraints, we have moved the detailed definition of \jensenDivergence in Appendix \ref{app:background}, as mentioned below:}\\
\changed{Jensen-Shannon Divergence or \jensenDivergence is used to realize the distance between two distributions. Specifically, it is computed by estimating the relative entropy between two distributions. The entropy of a random variable $X$ having probability mass function $P(x)$ is given as:

\begin{equation}
    H(X) = -\sum_{x \in X} P(x)log_{b}P(x)  \nonumber
\end{equation}

\jensenDivergence is estimated using the Kullback-Leibler divergence (KL-divergence). KL-divergence also measures the distance between two distributions. However, it is not symmetric and does not satisfy the triangle inequality. \jensenDivergence is an approach that improves upon the KL-divergence, as it is symmetric and a smoothed version of KL-divergence. KL divergence between two distributions $p$ and $q$ is given as:

\begin{equation}
    D_{KL}(p||q) = \int_{-\infty}^{\infty} p(x) log \left(\frac{p(x)}{q(x)}\right) dx  \nonumber 
\end{equation}

\jensenDivergence between two distributions $p$ and $q$ is given as:

\begin{equation}
    JSD(p||q) = \frac{1}{2} \left( D_{KL}(p||m) + D_{KL}(q||m) \right)  \nonumber
\end{equation}
}\\


\textbf{C3.} What is Jensen-Divergence like for benign models?
What is the detection criterion? In Figure 6: malicious models have a larger Jensen-divergence. In Figure 7: malicious models’ Jensen -divergence has a low variance. \\
\answer{We encountered two patterns of the malicious updates maximum \jensenDivergence values. First, malicious updates are either more significant than benign updates, or malicious updates are similar with variance low. Alternatively, it can be said that benign updates' maximum \jensenDivergence values did not differ significantly or were not similar. We discussed this in detail in R3 and R7.}\\


\textbf{C4.} The similarity between a client and clusters is used for filtering malicious models. It is observed that the similarity scores of malicious models are much higher than the benign clients. Can you explain this observation?  \\
\answer{We have discussed this R7.}\\

\textbf{C5.} Can adaptive attackers collude to form a cluster with a similar variation as the benign clusters. How can \ourname defend against this type of attack? \\
\answer{This comment was addressed by Major Revision requirement R6.}\\


\textbf{C6.} Can you show defensive performance against an attack that performs innocently and maliciously alternatively? An attacker, or a benign client might not follow a consistent distribution during the training process. We compute each client’s current distribution P (at time t) using the previous Iteration’s base measurement (at time t-1):
What if the attacker behaves normally before iteration (t-1) and suddenly begins to attack at iteration t.
What if a benign client also changes its distribution because of usage pattern change. \\
\answer{\begin{itemize}
    \item What if the attacker behaves normally before iteration ($t-1$) and suddenly begins to attack at iteration $t$.\\
    Yes, \ourname is able to defend against such strategies from malicious clients. We evaluated \ourname against such attacks. We ran the experiment for 3 rounds, having set the number of malicious clients (if any) to 6 out of a total of 30 clients. In the first two rounds, we set the number of malicious clients to zero, and in the third round, we introduced a mix of benign and malicious clients, having a total of 6 malicious clients and 24 benign clients. As shown in Figure~\ref{fig:htom_cifar} (below) in this document, the \jensenDivergence ($Max_{JD}^{i}$) of malicious updates in round 2 (starting from 0th index) differs greatly, thus \ourname was successful in preventing such attacks.
    
    \begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
     \centering
     \includegraphics[width=\textwidth ]{figures/honesttomalicious_PMR_610000.pdf}
     \caption{round = 0}
      \label{fig:htom_1}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.3\textwidth}
     \centering
     \includegraphics[width=\textwidth]{figures/honesttomalicious_PMR_610001.pdf}
     \caption{round = 1}
     \label{fig:htom_2}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.3\textwidth}
     \centering
     \includegraphics[width=\textwidth]{figures/honesttomalicious_PMR_610002.pdf}
     \caption{round = 2}
     \label{fig:htom_3}
    \end{subfigure}
    \caption{Jensen Divergence ($Max_{JD}^{i}$) for the CIFAR dataset, where the first two rounds do not contain any malicious clients, and the third round contains a mix of malicious and benign clients.}
    \label{fig:htom_cifar}\vspace{-0.3cm}
    \end{figure*}
    
    \item What if a benign client also changes its distribution because of usage pattern change. \\ 
    To answer this question, we assumed the same setup as in the previous question, except that in the first and the last round the number of malicious clients was set to zero, and in the second round a mix of benign and malicious clients was introduced (specifically, having a total of 6 malicious clients and 24 benign clients). Again, in this case, \ourname was successful in detecting malicious updates, as shown in Figure~\ref{fig:htom_cifar_alt} (below in this document).
    
    \begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
     \centering
     \includegraphics[width=\textwidth ]{figures/honesttomalicious_PMR_610000_alt.pdf}
     \caption{round = 0}
      \label{fig:htom_1_alt}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.3\textwidth}
     \centering
     \includegraphics[width=\textwidth]{figures/honesttomalicious_PMR_610001_alt.pdf}
     \caption{round = 1}
     \label{fig:htom_2_alt}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.3\textwidth}
     \centering
     \includegraphics[width=\textwidth]{figures/honesttomalicious_PMR_610002_alt.pdf}
     \caption{round = 2}
     \label{fig:htom_3_alt}
    \end{subfigure}
    \caption{Jensen Divergence ($Max_{JD}^{i}$) for the CIFAR dataset, where the first and the third round do not contain any malicious clients, and the second round contains a mix of malicious and benign clients.}
    \label{fig:htom_cifar_alt}\vspace{-0.3cm}
    \end{figure*}
    
\end{itemize}}

\textbf{C7.} Can you add a symbol definition table in the paper?\\
\answer{This comment was addressed by Major Revision requirement R9.}\\

\textbf{C8.} In fig. 9, I can not see the line of ‘No denfense MA.’ Does another line cover it? \\
\answer{Thanks for pointing this out! We have now fixed this in the paper. Please refer to Figure~\ref{fig:bd_nodefense} in the paper.}\\

\textbf{C9.} It is unclear when to assign the current client to an existing cluster and when to start a new cluster in the CRP clustering method. Does the ‘new cluster’ mean the client distribution itself? \\
\answer{Clients are being assigned to clusters according to $Max_{JD}^{i}$, as discussed in R9 (background adaptation).}

\subsection*{REVIEWER  D} 

\textbf{D1.} The argument that the defense's probabilistic method decouples the local client training from the global server's aggregation process is not correct. This is because such an argument implies that the probabilistic model makes the aggregated update independent of the local model updates (which the adversary controls). \\
\answer{This comment was addressed by Major Revision requirement R1.}\\

\textbf{D2.} Similarly, designing the defense around what is essentially a sampling process over the space of the client weights, does not mean that "the defense process becomes independent of the underlying local data distributions used for training."\\
\answer{This comment was addressed by Major Revision requirement R4 and Major Revision requirement R5.} \\

\textbf{D3.} It is not clear why the measure theory introduction is included. I found it to be rather confusing. I would have given an informal introduction to the Bayesian process and then formalize it properly in the appendix (if need be). \\
\answer{This comment was addressed by Major Revision requirement R9.}\\

\textbf{D4.} While the paper argues that it improves upon prior work removing the IID assumption, the exchangeability requirements of section 4 essentially amount to an order-independence assumption. As a result, the defense does not prevent attacks such as batch re-ordering.\\
\answer{In our work, we have not made any assumptions about the local clients' data. We are assuming that each client's update in each round is new data or new information. Also, the exchangeability assumption is with respect to the client's updates, not the client's data. Hence, even if an adversary launches the batch re-ordering attacks, it will not affect the working of \ourname.}\\

\textbf{D5.} Perhaps my largest issue with the paper is the presentation of the detection part of the algorithm; or lack thereof. There is very little explanation in the paper actually discussing the detection algorithm. The only direct discussion I have found is in "Filtering and Aggregation"  \\
\answer{This comment was addressed by Major Revision requirement R3.}\\
 
\textbf{D6.} It is unclear how these patterns are found; and how malicious ones are flagged. Is a thresholding mechanism in place on the likelihood of an update being from the same distribution, for example? This is such an important detail that I believe leaving it out is enough grounds for rejection. I like to point out that Section 5.3 and Algorithm 1 within also do not discuss the detection procedure details.\\
\answer{This comment was addressed by Major Revision requirement R3.}\\

\textbf{D7.} 
The paper emphasizes the decoupling of the defense from the client updates as the main motivation for using a probabilistic model; the actual models selected are not at all motivated. For example, it is not clear why a hierarchical model is needed. \\
\answer{ We use baseline Beta Process to compute Hierarchical Beta process for each client in an FL training round. The motivation behind using the Hierarchical Beta process, i.e., computation of the Beta Process for each client, is to keep track of the changes being made by each client in the computation of model updates. Ultimately, the update of the Beta Process parameters or the computation of Beta Process posteriors given the new client updates are then used in the detection phase to filter out the malicious updates.}\\

\textbf{D8.} I found the parameter definition for "non-iid" to be confusing. Overall, I find the "non-iid" to be a misnomer; because it is not inclusive of all forms of iid-ness. \\
\answer{We aligned our experimental setup, including this parameter (\nonIid) with recent work on poisoning attacks~\cite{nguyen22Flame,rieger2022deepsight}. The \nonIid parameter indicates the overlap of the data distributions of the individual clients. A \nonIid value of 0, therefore, completely \iid, indicates that all clients' data follow the same distribution, i.e., are independently and identically distributed. A \nonIid of 1.0 indicates that the data of clients (with different main labels) is heterogeneous, therefore, not identically distributed. We have clarified this in \sect\ref{subsec:ic} (Experimental Results), as follows:}\\
\changed{Following recent work~\cite{wang2020attack,fang2020local,rieger2022deepsight,nguyen22Flame}, we prepare the \nonIid data by varying the number of images assigned to a particular class for each client. Specifically, we form 10 groups corresponding to the ten classes of CIFAR-10. Then, clients in each group are allocated a fixed fraction of images, depending on the \nonIid degree of that group's label, while allocating the remaining images to each client at random.
%\mj{This sentence is not clear!}. 
In other words, for \nonIid = $0.0$ the samples of all clients follow the same distribution and were chosen randomly from all classes, while for \nonIid = $1.0$ the samples of each client were only chosen from the samples belonging to the main class of this client.}
%todoPhillip

==> 04_challenges.tex <==
\section{Requirements}
\label{sec:challenges}\vspace{-0.2cm}
%\commentA{WHy this section is defined as a requirements? }
%\kavita{In the initial version, we created a separate subsection for the challenges. But I removed it, as we already discussed the challenges in the introduction and it was taking extra space.}
%\commentA{This section needs more intuitive explanation of the formal stuff}
%\kavita{updated}
In this section, we discuss the requirements posed on \ourname due to the BNP nature of our defense. 
%\commentA{Where do you formulate the challenges in this section?}
In BNP models, exchangeability (defined below) is a critical requirement that must be satisfied by the sequence of random variables to model different parameters, such as priors and posteriors (see \sect\ref{sec:background}). 
\commentA{Are they satisfied in our FL model and why ? Argument informally why } 
\kavita{answered below}
Informally, the exchangeability property (of a sequence of random variables) states that the joint distribution of all the random variables remains the same for any permutation of random variables. 

In this work, we are modeling the client updates ($W_{i,l}$) and it's $l$ values as the detection module (CRP-Jensen) input data and the Hierarchical Beta-Bernoulli Process (HBBP), respectively. Thus, we consider both the client updates, $W_{i,l}$ and its $l$ values to satisfy the exchangeability property. Client updates or $W_{i,l}$ follow the exchangeability property because one client's local training is not dependent on another client's local training. Thus, permuting the client updates $W_{i,l}$ or changing the order of the incoming client updates will not affect the output of the detection module. Client $i$ update $l$ values also follow the exchangeability property because changing the order of client $i$'s update $l$ values won't affect the computation it's BP posterior $A_{i}$. The reason is, in Eq.\ref{eq_n:1}, we only utilize the summation of client $i$'s update $l$ values in the update of base measure $H_{i}$. 

We identify two essential requirements that will be used in the design of \ourname. 
%\commentA{I do not understnad this. You must aruge that the weights are exchangeable, i.e., this requirement is fulfilled.} \\

\noindent
\textbf{Requirement I. }\textit{For the posterior computation, a flattened  client weight is a sequence of random variables and should be drawn from an exchangeable set of choices.} 
%\commentA{define flattend at a high level in background section}

In posterior computation, we assume that the flattened client weight vector is a sequence of $l$ independent BeP draws,
%with success probability, $b_{i,l} = p_{w}^{h}$, if a weight $w$ is to be included in this vector
given the Beta prior, $A_{i}$. Thus, we consider that the $l$ values in a client weight vector $W_{i, l}$ are drawn from an exchangeable set of choices.
Mathematically, the sequence of the random variables, $X_{1}, X_{2}, ..., X_{l}$ is called an exchangeable sequence if the distribution of $X_{1}, X_{2}, ..., X_{l}$ is equal to the distribution of $X_{\pi_{1}}, X_{\pi_{2}}, ..., X_{\pi_{l}}$ for any permutation $(\pi_{1}, \pi_{2}, ..., \pi_{l})$. In other words, the joint distribution of all the random variables is the same for any permutation. We consider $W_{i, l} = ( W_{i, 1}, W_{i, 2}, ..., W_{i, l} )$ is an exchangeable sequence for the \mbox{computation of Beta posterior in \ourname.} 
%\commentA{Why is this assumption reasonable, exaplin}
\\

\noindent
\textbf{Requirement II. }\textit{For the CRP-Jensen based clustering mechanism, each client update is a sequence of random variables and should be drawn from an exchangeable set of choices.} 

CRP is an infinite mixture model which is used to assign data or samples to the mixtures (or clusters).
%\commentA{Is mixture a cluster here?}\kavita{mixtures are the clusters in mixture modeling}. 
%In infinite mixture modeling, the number of mixtures are not known beforehand, thus its non-parametric Bayesian approach to mixture modeling. 
The data or the samples are assumed to be drawn from an exchangeable set of choices. Hence, irrespective of the order in which the data arrives, their assignment to the mixtures or clusters (i.e., their seating arrangement in CRP) is not affected. Thus, in this work, we consider the incoming client updates, $W_{i, l}$, where $1 \leq i \leq n$ and $n$ is the number of clients, as a form of an exchangeable sequence. \\
%\commentA{You ar emaking assumptions about the distribution???}
%\kavita{not making any assumptions about the distribution type}
%-----------------------------------------------------------
%While modeling \ourname to defend against the backdoors in FL, we ascertained the following challenges:\\

%\noindent
%\textbf{Challenge I: Parametric Decoupling. }\textit{How to effectively compute a probabilistic measure that can be utilized to \changed{decouple} the detection algorithm of the designed defense from (i) the number of clients selected in each training round, (ii) the underlying data-distribution of each client, and (iii) the different attack strategies of an attacker?}

%It is tricky to design an effective defense mechanism against poisoned model updates as 
%Numerous factors can influence the accuracy of a backdoor defense mechanism. First, multiple clients are selected in a training round, and each client's data distribution is typically different; thus, the designed defense must be robust against the number of clients selected and their data distributions. In FL, by design, the global server is unaware of the training process executed on each client's side, and thus, a malicious client can evade anomaly detection by the global server by appropriately scaling its weights. Consequently, another important requirement from any defense mechanism against backdoor attacks in FL is that it should be robust against the weight update strategies employed by the attacker (malicious clients). We address the above challenges by computing a Beta posterior, given new client weights, s.t. the detection module of the defense can use this Beta posterior to filter out the malicious client updates without affecting the benign performance of the model. As outlined earlier, we employ a HBBP to compute each client's Beta posterior as a measure on their updates in order to resolve the above critical challenges. \\


%\noindent
%\textbf{Challenge II: High Performance.} \textit{How to design an effective algorithm for detecting malicious updates s.t. the benign performance of the global model is not adversely affected?} 


%The efficacy and efficiency of any defense mechanism against backdoor attacks in FL can be characterized by how well it is able to detect (and remove) all malicious updates, without limiting the benign performance of the target global model. Thus, it is imperative to distinguish malicious updates from benign updates. 
%To overcome this challenge, we designed \textit{CRP-Jensen}  to look for the patterns in the computed maximum \jensenDivergence metric (cf.~\sect\ref{subsubsec:filtering}), %\commentH{ Refer to the section where you define the metric}
%corresponding to each client, which can help distinguish the malicious updates from the benign updates.
%To overcome this challenge, we design a CRP-Jense based clustering technique which employs a maximum \jensenDivergence metric (cf.~\sect\ref{subsubsec:filtering}) to cluster and distinguish malicious updates from benign updates.

==> crp_jensen.tex <==
We first update the client's parameters using the beta posterior computed above using Hierarchical beta-Bernoulli process and is given as:

\begin{equation}
    W^{C}_{i, l} = x + cosine_s \quad \forall x \in W^{C}_{i, l} 
\end{equation}

where $cosine_s$ is the cosine angular distance computer between the local model and the global model. We then compute two probability distributions $p$ and $q$ and use Jensen-divergence to compute the similarity between them. $p$ represents the probability distribution of the clients computed using the updated based measure (described above) and $q$ represents the probability distribution of each of the clusters. Thus, for each client, we compute it's Jensen-divergence with each of the clusters $p$ (already formed and the new cluster as well). Then, we compute the max of this set of Jensen-divergences and decide which cluster the client's update belongs to. $p$ is computed in three steps:

$$p = \mathcal{N}(W^{C}_{i, l}; \mu_{p}, \sigma_{p})$$
$$p = x + (ubm) \quad \forall x \in p$$
\begin{equation}
    p = \mathcal{N}(p; 1, \overline{W^{C}_{i, l}})
\end{equation}


$q$ is computed as:
\begin{equation}
    q = \mathcal{N}(W^{C}_{i, l}; \mu_{c}, \sigma_{c})
\end{equation}


where, $\overline{W^{C}_{i, l}}$ is the mean of $W^{C}_{i, l}$, $\mu_{p}$ and $\sigma_{p}$ are the mean and the variance of initial global model respectively. $ubm$ is the updated base measure that is given as $\frac{c_{i}}{c_{i}+l} H + \frac{1}{c_{i} \times l} \sum_{i = 1}^{l}W^{C}_{i, l}$. $\mu_{c}$ and $sigma_{c}$ are mean and variance of the clusters, respectively.

After computing the cluster of the client update, we update the mean and the variance of that particular cluster according to the formula:

\begin{equation}
    \mu_{new} = \frac{\overline{W^{C}_{i, l}} n_{k} \tau_{k}+ \mu_{0} \tau_{0}}{n_{k} \tau_{k}+ \tau_{0}} 
\end{equation}

\begin{equation}
    \sigma_{new} = \frac{1}{n_{k}\tau_{k}+ \tau_{0}} + \sigma_{y}^{2} 
\end{equation}

where, $n_{k}$ is the number of client update already assigned to it, $\tau_{k}$ represents the precision of the cluster, $\mu_{0}$ and $\tau_{0}$ represents the initial mean and the precision assumed for the new clusters. $\sigma_{y}^{2}$ is the variance due to the measurement introduced by the new addition of the client updates and is compute as: $\sigma_{y}^{2} = dist_{norm}$. $dist_{norm}$ is the euclidean distance between the local model update and the global model. We will now outline the mixture model clustering algorithm to filter out the poisoned updates.  
\vfill
\pagebreak


